VortSDF: 3D Modeling with Centroidal Voronoi Tesselation on Signed Distance Field

Volumetric shape representations have become ubiquitous in multi-view reconstruction tasks. They often build on regular voxel grids as discrete representations of 3D shape functions, such as SDF or radiance fields, either as the full shape model or as sampled instantiations of continuous representations, as with neural networks. Despite their proven efficiency, voxel representations come with the precision versus complexity trade-off. This inherent limitation can significantly impact performance when moving away from simple and uncluttered scenes. In this paper we investigate an alternative discretization strategy with the Centroidal Voronoi Tesselation (CVT). CVTs allow to better partition the observation space with respect to shape occupancy and to focus the discretization around shape surfaces. To leverage this discretization strategy for multi-view reconstruction, we introduce a volumetric optimization framework that combines explicit SDF fields with a shallow color network, in order to estimate 3D shape properties over tetrahedral grids. Experimental results with Chamfer statistics validate this approach with unprecedented reconstruction quality on various scenarios such as objects, open scenes or human.

==> Sections/Backup.tex <==
%The 3D surface is represented as the zero crossing of a signed distance field (SDF) that is explicitly discretized on a hierarchical CVT. Another CVT grid with the same shape contains learnable features. Two shallow MLPs are used to predict view dependent color at each point in the 3D space. Following \cite{voxurf} the coarse network $g_{geo}$ takes as input, 3D position, ray direction and explicit features defined from the SDF field. Differently from \cite{voxurf} we propose a new geometric features that is best adapted to a tetrahedral grid. The fine color network $g_{fine}$ takes as input position, ray direction, coarse color and 6D learnable features. The color of a point in 3D for final rendering is the output of $g_{fine}$ but the photometric error is backpropagated for both networks. Our goal is to optimize the weights color networks, the learnable features and the values of the sdf tetrahedral grid given a set of multi-view images ${I_k}_{k \in[1:N]}$.Figure \ref{fig::pipeline} illustrates the pipeline of our proposed method. 

%The 3D surface is represented as the zero crossing of a signed distance field (SDF) that is explicitly discretized on a hierarchical CVT. Another CVT grid with the same shape contains learnable features. Two shallow MLPs are used to predict view dependent color at each point in the 3D space. Following \cite{voxurf} the coarse network $g_{geo}$ takes as input, 3D position, ray direction and explicit features defined from the SDF field. Differently from \cite{voxurf} we propose a new geometric features that is best adapted to a tetrahedral grid. The fine color network $g_{fine}$ takes as input position, ray direction, coarse color and 6D learnable features. The color of a point in 3D for final rendering is the output of $g_{fine}$ but the photometric error is backpropagated for both networks. Our goal is to optimize the weights color networks, the learnable features and the values of the sdf tetrahedral grid given a set of multi-view images ${I_k}_{k \in[1:N]}$.

%For a color network $g$ that can be either $g_{geo}$ or $g_{fine}$ the rendered color at pixel $(i,j)$ is:
%\begin{align}
%    V_{\Theta}: \R^3 \to \R^4 \\
%    x \to (sdf(x), c(x)).
%\end{align}

%Our goal is to optimize the weights $\Theta$ of the neural field given a set of multi-view images ${I_k}_{k \in[1:N]}$.

%With the network $V_{\Theta}$ an image ${I_k}_{k \in[1:N]}$ is rendered for a camera pose by using a ray tracing algorithm. A ray is shot from the center of the camera to each pixel in the image plane. Points are sampled along the ray and the sdf and color values at these 3D points are obtained from the surrounding sites of the CVT. The color at the pixel is computed by integrating the color values weighted by a function that depends on the sdf value. 


Level-set approaches are efficient methods for 3D reconstruction with strong mathematical foundations. Originally, level-set methods were defined to fit an input set of range images. We reformulate the level set solutions for input multi-view images and hybrid implicit neural models of the (colored) 3D shape.

Let $S$ be the 3D surface that encloses the object. Let ${I^{(1)}, ...I^{(n)}}$ be a set of input images. The posterior probability of $S$ is given by Bayes rule:
\begin{equation}
    P(S|I^{(1)},...I^{(n)}) = \frac{P(I^{(1)},...I^{(n)}|S)P(S)}{P(I^{(1)},...I^{(n)})}.
\end{equation}

Our goal is to find most likely surface model $S$ that would be rendered similar to a particular collection of images,
\begin{equation}
    \sup_S[P(S|I^{(1)},...I^{(n)})] = \sup_S[P(I^{(1)},...I^{(n)}|S)P(S)].
\end{equation}
The denominator can be dropped because it does not depends on the surface S and thus does not impact the optimization result. The term $P(S)$ is the prior term, which reflects that some surfaces are most likely than others (like smooth surfaces).

The images, conditioned on the surface geometry are independent random variables.
\begin{equation}
    P(I^{(1)},...I^{(n)}|S) = \prod_i P(I^{(i)}|S).
\end{equation}
Each image consists of an array of pixels that can be represented as $r_{u,v}^{(i)}$. Within an image each pixel is an independent random variable, and therefore
\begin{equation}
    P(I^{(1)},...I^{(n)}|S) = \prod_i \prod_{u,v} P(r_{u,v}^{(i)}|S).
\end{equation}

As is typical with MAP algorithms, the maximization is performed as a minimization on the negative logarithm of the probability:
\begin{align}
    \sup_S[P(S|I^{(1)},...I^{(n)})] = \\ \inf_S\left\{ - \sum_i \sum_{u,v} \ln P(r_{u,v}^{(i)}|S) -\ln P(S) \right\}.
\end{align}

\subsubsection{The data term}
Each individual pixel measurement is dependent not on the surface $S$ as a whole, but on a particular point on the surface that intersects with the line of sight. With modern differentiable rendering technology, the pixel measurement $r_i$ depends on an integral along its associated line of sight. Following differentiable rendering formulation as in NeUS and the Gaussian noise model gives the following probability function for individual pixel readings,
\begin{align}
    -\ln P(r_i|S) = \frac{1}{\sigma_i^2}(c_i - r_i)^2 + \frac{1}{\sqrt{w\pi\sigma}} \\ = \alpha_i(c_i - r_i)^2 + \kappa(\alpha_i).
\end{align}
The term $\kappa(\alpha_i)$ can be ignored because it does not depend on the surface geometry.

The color $c_i$ is obtained with the discrete integration along the line of sight:
\begin{flalign}
    c_i = \sum_{t=0}^{n}{\omega(t|S)C(p(d_t), v)}, \\
    \label{eq::render}
    \omega(t|S) = \alpha(t|S)T(t|S), \\
    T(t|S) = \prod_{i < t}(1-\alpha_i(S)).
\end{flalign}

%For a surface $S$ let $I_S$ be the function that is $1$ inside (surface included) and $-1$ outside. Similarly let $\Tilde{I}_S$ be the function that is $1$ outside the surface (surface included) and $-1$ inside. Then we can write
For a surface $S$ let $\Omega$ be inside and $\Bar{\Omega}$ outside. Then we can write
\begin{align}
    c_i = \int_{\Omega} c(x) \alpha(x)T(x)dx + \\ \int_{\Bar{\Omega}} c(x) \alpha(x)T(x)dx
\end{align}

Then,
\begin{align}
    -\ln P(r_i|S) \simeq \alpha_i(\int_{\Omega} c(x) \alpha(x)T(x)dx + \\ \int_{\Bar{\Omega}} c(x) \alpha(x)T(x)dx - r_i)^2+ \kappa(\alpha_i).
\end{align}

We can now write the derivatives of the surface as follows:
\begin{align}
    \frac{\partial S}{\partial t} = 2(c_i - r_i)\dfrac{\partial}{ \partial t}([c(S) \alpha(S)T(S)N - \\ c(S) \alpha(S)T(S)(-N)]). \\
                = 4(c_i - r_i)\dfrac{ \partial}{\partial t} (c(S)\alpha(S)T(S)) N.
\end{align}

The effect of all pixels is additive, and the posterior can be combined to obtain:
\begin{align}
    \frac{\partial S}{\partial t} = -g(S) N + \rho(S), \\
    g(S) = 2\sum_i(c_i - r_i)\frac{ \partial}{\partial t} (c(S)\alpha(S)T(S)).
\end{align}

\subsubsection{The prior term}
We follow previous works to write the prior smoothness using mean curvature.
\begin{align}
    \rho(S) = (\frac{\partial^2 S}{\partial u^2} + \frac{\partial^2 S}{\partial v^2}).
\end{align}
%\begin{align}
%    \rho(S) = (\beta + \lambda) (\frac{\partial^2 S}{\partial x^2} + \frac{\partial^2 S}{\partial y^2}) + \\
%    (\beta \lambda)(\frac{\partial^4 S}{\partial x^4} + \frac{\partial^4 S}{\partial y^4}).
%\end{align}
Where $u$ and $v$ are the surface parameters.

\subsubsection{Level set model}
We represent the surface $S$ with a function $\phi$ such that:
\begin{align}
    S(t) = \{x | \phi(x,t)=0\}.
\end{align}

The surface $S$ remains a level set of $\phi$ over time, and therefore the time derivative is zero:
\begin{align}
    \frac{\partial \phi(S,t)}{\partial t} + \nabla \phi(S,t) \cdot \frac{\partial S}{\partial t}.
\end{align}

Thus, 
\begin{align}
    \frac{\partial \phi}{\partial t} = -\nabla \phi \cdot \frac{\partial S}{\partial t} = |\nabla \phi|\frac{\partial S}{\partial t} N.
\end{align}
%\begin{align}
%    \frac{\partial \phi}{\partial t} = -\nabla \phi \cdot \frac{\partial S}{\partial t} = |\nabla \phi|\frac{\partial S}{\partial t} N \\
%            =|\nabla \phi|(g(x) + ((\beta + \lambda) \Delta \phi + \\
%    (\beta \lambda)(\frac{\partial^4 \phi}{\partial x^4} + \frac{\partial^4 \phi}{\partial y^4})) \cdot N.
%\end{align}


We represent the surface $S$ with a function $\phi$ such that:
\begin{align}
    S(t) = \{x | \phi(x,t)=0\}.
\end{align}

We assume that the surface $S$ remains a level set of $\phi$ over time, and therefore the time derivative is zero:
\begin{align}
    \frac{\partial \phi(S,t)}{\partial t} + \nabla \phi(S,t) \cdot \frac{\partial S}{\partial t} = 0.
\end{align}

Thus, 
\begin{align}
    \frac{\partial \phi}{\partial t} = -\nabla \phi \cdot \frac{\partial S}{\partial t} = |\nabla \phi|\frac{\partial S}{\partial t} N,
\end{align}
where $\nabla \phi|$ is the spatial gradient of the SDF values and $N$ is the unit normal vector of the SDF field.


A common problem in previous works such as Voxurf \cite{voxurf} is the trade-off between smoothness and ability to capture fine details. Our key idea is to re-formulate the optimization process so that the surface evolves in the direction of the normal vectors. In addition, we propose to use the Taubin function for the smoothness constraint instead of the mean curvature loss \cite{NeuralAngelo}, which is able to smooth the surface while keeping sharp details.




\begin{table*}[t]
    \centering
    \caption{Average Chamfer distances (cm), normal consistency (lower is better) and PSNR errors obtained for both Our proposed method and NeuS for each of the $8$ test scenes. We also compare the quality of the output meshes when using Marching Cubes (MC) or clipped CVT (CVT)}
    %\vspace*{3mm}
    \begin{tabular}{|c||c|c|c||c|c|c||c|c|c|}%|c|}
    \hline
     & \multicolumn{3}{|c||}{NeuS} & \multicolumn{3}{|c||}{Voxurf} & \multicolumn{3}{|c|}{Ours}  \\
    \hline
     & Chmf & PSNR & Time & Chmf & PSNR & Time  & Chmf & PSNR & Time   \\
    \hline
     Dog & $?$ & $24.77(21.87)$ & $8$h$30$ & $?$ & $\mathbf{30.00}$ & $30$mn & $\mathbf{?}$ ($?$) & $27.03$  & $?$\\
     \hline
     Bear & $?$ & $24.15(20.33)$ & $8$h$30$ & $?$ & $24.16$ & $?$ & $?$ ($\mathbf{?}$) & $\mathbf{24.85}$ & $?$\\
     \hline
     Clock & $?$ & $16.84(17.21)$ & $8$h$30$ & $?$ & $\mathbf{25.90}$ & $?$ & $\mathbf{0?}$ ($?$) & $25.40$ & $?$\\
     \hline
     Durian & $?$ & $15.96(23.03)$ & $8$h$30$ & $?$ & $22.57$ & $30$mn & $\mathbf{?}$ ($?$) & $\mathbf{23.61}$  & $?$\\
     %\hline
     %Jade & $?$ & $\mathbf{15.8}$ & $?$ & $27.91$ & $?$ & $?$ & $?$  \\
     \hline
     Man & $19.4$ & $32.62(29.36)$ & $8$h$30$ & $13.1$ &  & $?$ & $\mathbf{7.0}$ ($7.1$) & $\mathbf{34.73}$ & $?$\\
     \hline
     Sculpture & $0.9$ & $29.03$ & $8$h$30$ &  $0.2$ & $\mathbf{31.69}$ & $?$ & $\mathbf{0.1}$ ($0.6$) & $29.60$ & $?$\\
     \hline
     Stone & $?$ & $23.40$ & $8$h$30$ & $?$ & $\mathbf{25.74}$ & $30$mn & $?$ ($\mathbf{?}$) & $24.41$ & $?$\\
     
    \hline
    \hline
     Avg & $?$ & $23.82$ & $8$h$30$ & $?$ & $26.38$ & $?$ & $?$ ($\mathbf{?}$) & $\mathbf{27.09}$ & $?$ \\
    
    
    \hline
    \end{tabular}
    \label{tab:chamferchmf}
\end{table*}


\begin{table*}[t]
    \centering
    \caption{Ablation study}
    %\vspace*{3mm}
    \begin{tabular}{|c||c|c||c|c||c|c||c|c||c|c|}%|c|}
    \hline
     & \multicolumn{2}{|c||}{w/ CVT} & \multicolumn{2}{|c||}{Lvl 1} & \multicolumn{2}{|c||}{Lvl 2} & \multicolumn{2}{|c|}{Lvl 3} & \multicolumn{2}{|c|}{Lvl 4}\\
    \hline
     & Acc & PSNR & Acc & PSNR & Acc & PSNR & Acc & PSNR & Acc & PSNR \\
    \hline     
    \hline
    \hline
     BMVS Man & $?$ & $31.08$ & $5.73$ & $26.21$ & $3.27$ & $28.37$ & $2.51$ & $30.12$ & $2.01$ & $34.73$ \\
    \hline
     Time & \multicolumn{2}{|c||}{$45$mn} & \multicolumn{2}{|c||}{$8$mn} & \multicolumn{2}{|c||}{$18$mn} & \multicolumn{2}{|c||}{$32$mn} & \multicolumn{2}{|c|}{$1$h}\\
    
    
    \hline
    \end{tabular}
    \label{tab:abla}
\end{table*}

==> Sections/CVTReview.tex <==
A tessellation of a 3D space is a disjoint set of polyhedron that fills the 3D space of interest. Centroidal Voronoi Tesselation (CVT) are used in a wide range of applications in Computer Graphics as it provides an elegant tool to compute a regular and optimized discretization of the 3D space \cite{wang:hal-01185210}. Voronoi tessellation is the dual of the Delaunay triangulation and is defined by its sites: a set of 3D points in space.

A Voronoi cell $V_i$ is associated with its site $x_i$ and consists of all points in space that are closest to $x_i$: \\ 
\begin{equation*}
    \{ p \in \ R^3 \ / \ ||p-x_i|| < ||p-x_j||, \ j \in [1,K], j\ !=\ i\}
\end{equation*}

%Or more generally 
%\begin{equation*}
%    \{ p \in \ R^3 / d(p,x_i) < d(p,x_j), \ j \in [1,K], \ j \ != \ i\} 
%\end{equation*}

%The set $\{ {V_i}\ ,i\in [1,K]\}$ defines a tessellation of the space of interest (a subspace of $R^3$). This tessellation is called Voronoi tessellation or Voronoi Diagram. Each cell is associated with its corresponding site $x_i$.

The bisector $B(i,j)$ of two sites $x_i$ and $x_j$ is the set of points $\{p \in R^3 / \ d(p,x_i) = d(p,x_j)\}$. In 2D it is a line, in 3D it is a plane. The bisector of multiple sites is the intersection between the bisectors of the pairs of sites. In 2D this creates segments. In 3D this creates polygons that can be subdivided into triangles. Each site $i$ is associated with a set of bisectors ${B_i}$ that represents a polygon and is composed of triangles. This also can be understood as the flat membrane that separates two sites. When each site of a Voronoi tessellation coincides with the centroid of its associated cell, the tessellation is called a Centroidal Voronoi Tessellation (CVT).

%There are two popular algorithms to optimize the positions of the sites to obtain a uniform CVT given initial positions: The LLoyd algorithm, which is an expectation maximization algorithm and the L-BFGS algorithm \cite{liu2009centroidal}, which is a quasi-newton optimization method. We choose the LLoyd algorithm in this paper because of its potential to be parallelized on the GPU. The Lloyd algorithm resembles a K-means algorithm where the sites are iteratively re-positionned at the center of the cells, the cells are then updated with the new positions of the sites.

%Figure\ref{fig::cvt} shows some example results of CVT computed for different shapes. As we can see from these results uniform CVT provide regular and detailed tessellation of a 3D volume.

%In the case of uniform density, computing the center of mass of each cell from the convex polyhedron that defines it can be done relatively easily by using existing tools for fast and accurate computation of polyhedral mass properties. For example Mirtich \cite{mirtich1996fast} proposed an algorithm that is based on a three step reduction of the volume integrals to successively simpler integrals. However, the case of non-uniform densities is extremely more difficult and each algorithm must adapt to the shape of the density function. In this paper we propose a approximation for the optimisation that is simple to implement and accurate.

\subsection{Clipped CVT}
Given a CVT and an sdf field, the 3D mesh of the $0$ level set can be extracted with clipping the CVT
\cite{Lee}. In short the process of clipping a CVT consists in (1) identifying edges of the bisectors that cross the $0$ level set; (2) Add new points in these edges that are at $0$ level set; (3) remove vertices that are outside the surface and re-triangulate each cell. The final 3D mesh is obtained as the surface of the clipped CVT.  
